Identification of Driver Phone Usage Violations via State-of-the-Art Object Detection with Tracking

The use of mobiles phones when driving have been a major factor when it comes to road traffic incidents and the process of capturing such violations can be a laborious task. Advancements in both modern object detection frameworks and high-performance hardware has paved the way for a more automated approach when it comes to video surveillance. In this work, we propose a custom-trained state-of-the-art object detector to work with roadside cameras to capture driver phone usage without the need for human intervention. The proposed approach also addresses the issues caused by windscreen glare and introduces the steps required to remedy this. Twelve pre-trained models are fine-tuned with our custom dataset using four popular object detection methods: YOLO, SSD, Faster R-CNN, and CenterNet. Out of all the object detectors tested, the YOLO yields the highest accuracy levels of up to 96% (AP10) and frame rates of up to ~30 FPS. DeepSort object tracking algorithm is also integrated into the best-performing model to collect records of only the unique violations, and enable the proposed approach to count the number of vehicles. The proposed automated system will collect the output images of the identified violations, timestamps of each violation, and total vehicle count. Data can be accessed via a purpose-built user interface.

==> r.tex <==
@misc{r1,
  author = {World Health Organization},
  title = {{Road traffic injuries}},
  howpublished = {\url{https://www.who.int/news-room/fact-sheets/detail/road-traffic-injuries}},
  year = {2021}, 
  note = "[Online; accessed 5-July-2021]"
}

@misc{r2,
  author = {GOV UK},
  title = {{Using a phone or a sat nav when driving}},
  howpublished = {\url{https://www.gov.uk/using-mobile-phones-when-driving-the-law}}, 
  year = {2021}, 
  note = "[Online; accessed 5-July-2021]"
}

@misc{r3,
  author = {GOV UK},
  title = {{Double penalties for motorists using mobiles}},
  howpublished = {\url{https://www.gov.uk/government/news/double-penalties-for-motorists-using-mobiles}}, 
  year = {2017}, 
  note = "[Online; accessed 7-July-2021]"
}

@article{r4,
title = {Mobile phone use while driving: A hybrid modeling approach},
journal = {Accident Analysis & Prevention},
volume = {78},
pages = {73-80},
year = {2015},
issn = {0001-4575},
doi = {https://doi.org/10.1016/j.aap.2015.02.016},
url = {https://www.sciencedirect.com/science/article/pii/S0001457515000573},
author = {Luis Márquez and Víctor Cantillo and Julián Arellana},
keywords = {Mobile phone, Phoning while driving, Distracted driving, Latent variable models, Hybrid modeling}
}

@article{r5,
  title={A deep learning approach to building an intelligent video surveillance system},
  author={Xu, Jie},
  journal={Multimedia Tools and Applications},
  volume={80},
  number={4},
  pages={5495--5515},
  year={2021},
  publisher={Springer}
}

@inproceedings{r6,
  title={Driver Cell Phone Usage Violation Detection using License Plate Recognition Camera Images},
  author={Alkan, Bensu and Balci, Burak and Elihos, Alperen and Artan, Yusuf},
  booktitle={VEHITS},
  pages={468--474},
  year={2019}
}

@inproceedings{r7,
  title={Multiple scale faster-rcnn approach to driver's cell-phone usage and hands on steering wheel detection},
  author={Hoang Ngan Le, T and Zheng, Yutong and Zhu, Chenchen and Luu, Khoa and Savvides, Marios},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition workshops},
  pages={46--53},
  year={2016}
}

@inproceedings{r8,
  title={Vehicle tracking using deep sort with low confidence track filtering},
  author={Hou, Xinyu and Wang, Yi and Chau, Lap-Pui},
  booktitle={2019 16th IEEE International Conference on Advanced Video and Signal Based Surveillance (AVSS)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@article{r9,
  title={Yolov3: An incremental improvement},
  author={Redmon, Joseph and Farhadi, Ali},
  journal={arXiv preprint arXiv:1804.02767},
  year={2018}
}

@article{r10,
  title={Yolov4: Optimal speed and accuracy of object detection},
  author={Bochkovskiy, Alexey and Wang, Chien-Yao and Liao, Hong-Yuan Mark},
  journal={arXiv preprint arXiv:2004.10934},
  year={2020}
}

@inproceedings{r11,
  title={End-to-end training of object class detectors for mean average precision},
  author={Henderson, Paul and Ferrari, Vittorio},
  booktitle={Asian Conference on Computer Vision},
  pages={198--213},
  year={2016},
  organization={Springer}
}

@article{r12,
  title={Transfer learning using vgg-16 with deep convolutional neural network for classifying images},
  author={Tammina, Srikanth},
  journal={International Journal of Scientific and Research Publications (IJSRP)},
  volume={9},
  number={10},
  pages={143--150},
  year={2019}
}

@mastersthesis{r13,
  title={Driver Handheld Cell Phone Usage Detection},
  author={Elings, Jannes W},
  year={2018}
}

@article{r14,
  title={YOLOv3: An Incremental Improvement. University of Washington},
  author={Redmon, Joseph and Farhadi, Ali},
  journal={arXiv preprint arXiv:1804.02767},
  year={2018}
}

@article{r15,
  title={Object detection in sports: TensorFlow Object Detection API case study},
  author={Mustamo, Pirkko},
  journal={University of Oulu},
  year={2018}
}


@misc{r16,
  author = {Tensorflow},
  title = {TensorFlow 2 Detection Model Zoo},
  howpublished = {\url{https://github.com/tensorflow/models/blob/master/research/object_detection/g3doc/tf2_detection_zoo.md }}, 
  year = {2021}, 
  note = "[Online; accessed 5-May-2021]"
}

@misc{r17,
  author = {Saxena, P},
  title = {{How to Label Images for Object Detection, Step by Step.}},
  howpublished = {\url{https://towardsdatascience.com/how-to-label-images-for-object-detection-step-by-step-7ee317f98583}}, 
  year = {2020}, 
  note = "[Online; accessed 30-March-2021]"
}

@inproceedings{r18,
  title={Microsoft coco: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={European conference on computer vision},
  pages={740--755},
  year={2014},
  organization={Springer}
}

@article{r19,
  title={Faster r-cnn: Towards real-time object detection with region proposal networks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  journal={Advances in neural information processing systems},
  volume={28},
  pages={91--99},
  year={2015}
}

@inproceedings{r20,
  title={Research on SSD base network},
  author={Kang, Yixuan},
  booktitle={IOP Conference Series: Materials Science and Engineering},
  volume={768},
  number={7},
  pages={072031},
  year={2020},
  organization={IOP Publishing}
}

@inproceedings{r21,
  title={CenterNet Heatmap Propagation for Real-Time Video Object Detection},
  author={Xu, Zhujun and Hrustic, Emir and Vivet, Damien},
  booktitle={European Conference on Computer Vision},
  pages={220--234},
  year={2020},
  organization={Springer}
}

@article{r22,
  title={Performance analysis of google colaboratory as a tool for accelerating deep learning applications},
  author={Carneiro, Tiago and Da N{\'o}brega, Raul Victor Medeiros and Nepomuceno, Thiago and Bian, Gui-Bin and De Albuquerque, Victor Hugo C and Reboucas Filho, Pedro Pedrosa},
  journal={IEEE Access},
  volume={6},
  pages={61677--61685},
  year={2018},
  publisher={IEEE}
}

@inproceedings{r23,
  title={Ssd: Single shot multibox detector},
  author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C},
  booktitle={European conference on computer vision},
  pages={21--37},
  year={2016},
  organization={Springer}
}

@inproceedings{r24,
  title={A delay metric for video object detection: What average precision fails to tell},
  author={Mao, Huizi and Yang, Xiaodong and Dally, William J},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={573--582},
  year={2019}
}

@article{r25,
  title={Wider or deeper: Revisiting the resnet model for visual recognition},
  author={Wu, Zifeng and Shen, Chunhua and Van Den Hengel, Anton},
  journal={Pattern Recognition},
  volume={90},
  pages={119--133},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{r26,
  title={Inception-v3 for flower classification},
  author={Xia, Xiaoling and Xu, Cui and Nan, Bing},
  booktitle={2017 2nd International Conference on Image, Vision and Computing (ICIVC)},
  pages={783--787},
  year={2017},
  organization={IEEE}
}

@article{r27,
  title={A novel image classification approach via dense-MobileNet models},
  author={Wang, Wei and Li, Yutao and Zou, Ting and Wang, Xin and You, Jieyu and Luo, Yanhong},
  journal={Mobile Information Systems},
  volume={2020},
  year={2020},
  publisher={Hindawi}
}

@misc{r28,
  author = {Shivy Yohanandan},
  title = {{mAP (mean Average Precision) might confuse you!}},
  howpublished = {\url{https://towardsdatascience.com/map-mean-average-precision-might-confuse-you-5956f1bfa9e2}}, 
  year = {2020}, 
  note = "[Online; accessed 7-July-2021]"
}

@misc{r29,
  author = {Ren Jie Tan},
  title = {{Breaking Down Mean Average Precision (mAP)}},
  howpublished = {\url{https://towardsdatascience.com/breaking-down-mean-average-precision-map-ae462f623a52}}, 
  year = {2019}, 
  note = "[Online; accessed 20-July-2021]"
}

@article{r30,
  title={The pascal visual object classes (voc) challenge},
  author={Everingham, Mark and Van Gool, Luc and Williams, Christopher KI and Winn, John and Zisserman, Andrew},
  journal={International journal of computer vision},
  volume={88},
  number={2},
  pages={303--338},
  year={2010},
  publisher={Springer}
}

@book{r31,
  title={Introducing Microsoft Power BI},
  author={Ferrari, Alberto and Russo, Marco},
  year={2016},
  publisher={Microsoft Press}
}

@incollection{r32,
  title={Times of crises and the development of the Police National Automatic Number Plate Recognition system in the UK},
  author={Norris, Clive and L’Hoiry, Xavier},
  booktitle={Big Data, Surveillance and Crisis Management},
  pages={198--221},
  year={2017},
  publisher={Routledge}
}

@article{r33,
  title={The open images dataset v4},
  author={Kuznetsova, Alina and Rom, Hassan and Alldrin, Neil and Uijlings, Jasper and Krasin, Ivan and Pont-Tuset, Jordi and Kamali, Shahab and Popov, Stefan and Malloci, Matteo and Kolesnikov, Alexander and others},
  journal={International Journal of Computer Vision},
  volume={128},
  number={7},
  pages={1956--1981},
  year={2020},
  publisher={Springer}
}

@article{r34,
  title={Deep learning-based multiple object visual tracking on embedded system for iot and mobile edge computing applications},
  author={Blanco-Filgueira, Beatriz and Garcia-Lesta, Daniel and Fern{\'a}ndez-Sanjurjo, Mauro and Brea, V{\'\i}ctor Manuel and L{\'o}pez, Paula},
  journal={IEEE Internet of Things Journal},
  volume={6},
  number={3},
  pages={5423--5431},
  year={2019},
  publisher={IEEE}
}

@article{r35,
  title={Light-head r-cnn: In defense of two-stage object detector},
  author={Li, Zeming and Peng, Chao and Yu, Gang and Zhang, Xiangyu and Deng, Yangdong and Sun, Jian},
  journal={arXiv preprint arXiv:1711.07264},
  year={2017}
}

@article{r36,
  title={Detection of masses in mammograms using a one-stage object detector based on a deep convolutional neural network},
  author={Jung, Hwejin and Kim, Bumsoo and Lee, Inyeop and Yoo, Minhwan and Lee, Junhyun and Ham, Sooyoun and Woo, Okhee and Kang, Jaewoo},
  journal={PloS one},
  volume={13},
  number={9},
  pages={e0203355},
  year={2018},
  publisher={Public Library of Science San Francisco, CA USA}
}

@book{r37,
  title={Foundations of machine learning},
  author={Mohri, Mehryar and Rostamizadeh, Afshin and Talwalkar, Ameet},
  year={2018},
  publisher={MIT press}
}

@book{r38,
  title={Deep learning},
  author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  year={2016},
  publisher={MIT press}
}

@misc{r39,
  title={Efficient inference with tensorrt},
  author={Vanholder, Han},
  year={2016},
  publisher={ed}
}

@article{r40,
  title={Statistics and Machine Learning in Python},
  author={Duchesnay, Edouard and Lofstedt, Tommy and Younes, Feki},
  year={2020}
}

@article{r41,
  title={Performance evaluation of object detection algorithms for video surveillance},
  author={Nascimento, Jacinto C and Marques, Jorge S},
  journal={IEEE Transactions on Multimedia},
  volume={8},
  number={4},
  pages={761--774},
  year={2006},
  publisher={IEEE}
}

@misc{r42,
  author = {Carrell},
  title = {Identification of Driver Phone Usage Violations using YOLOv4, YOLOv3 and DeepSort},
  howpublished = {\url{https://github.com/carrell-ncl/Windscreen2}}, 
  year = {2021}, 
  note = "[Online; accessed 19-August-2021]"
}
